Fully GPU-accelerated semistochastic Epstein-Nesbet perturbation theory

Second-order Epstein-Nesbet perturbation theory (EN-PT2) is an important tool for improving selected configuration interaction (SCI) energies, but the large external determinant space creates substantial memory and communication costs on GPU clusters. We develop a fully GPU-accelerated implementation of distributed semistochastic EN-PT2, fusing excitation generation, screening, and PT2 weighting in a single kernel traversal. Fixed-size random-phase CountSketch arrays limit memory use and replace large external determinant exchange with bounded collective summation. The implementation on one A100 completes EN-PT2 calculations 8.21-37.53 times faster than Arrow on 64 CPU cores at the same requested statistical standard error, and fixed-workload strong-scaling tests achieve 93.5% parallel efficiency on 16 GPUs across two nodes. Applications to an iron-oxo complex in a (60e, 187o) active space, iron-porphyrin references containing 200 million determinants per state, and neural-network quantum states establish the method's efficiency for perturbative corrections to large reference wave functions in the GPU era.

==> assets/qiankunnet-logo-paths.tex <==
% Exact vector contours from the user-supplied VI v0.3 outlined SVG.
% Units are those of the master: cap height 28; baseline y=0.
% No font file, raster artwork or shell escape is required.
\fill[QKBrandPrimary] (0,23.2) rectangle (36,28);
\fill[QKBrandPrimary] (0,11.6) rectangle (36,16.4);
\fill[QKBrandPrimary] (0,8.88178e-16) rectangle (36,4.8);
\fill[QKBrandSecondary] (42,23.2) rectangle (57,28);
\fill[QKBrandSecondary] (42,11.6) rectangle (57,16.4);
\fill[QKBrandSecondary] (42,8.88178e-16) rectangle (57,4.8);
\fill[QKBrandSecondary] (63,23.2) rectangle (78,28);
\fill[QKBrandSecondary] (63,11.6) rectangle (78,16.4);
\fill[QKBrandSecondary] (63,8.88178e-16) rectangle (78,4.8);
\path[fill=QKBrandPrimary]
  (105.53757225435,26.74566473991)
  .. controls (111.40462427748,26.74566473991) and (112.13294797690,19.17919075146) .. (112.21387283239,14.00000000001)
  .. controls (112.13294797690,8.49710982660) and (111.40462427748,1.25433526012) .. (105.53757225435,1.25433526012)
  .. controls (99.67052023122,1.25433526012) and (98.94219653180,8.49710982660) .. (98.86127167631,14.00000000001)
  .. controls (98.94219653180,19.17919075146) and (99.67052023122,26.74566473991) .. (105.53757225435,26.74566473991)
  -- cycle
  (105.53757225435,28.60693641621)
  .. controls (96.23121387284,28.60693641621) and (91.69942196532,23.14450867054) .. (91.69942196532,14.00000000001)
  .. controls (91.69942196532,5.66473988440) and (95.50289017342,0.40462427746) .. (103.10982658961,-0.44508670520)
  .. controls (104.24277456649,-3.35838150289) and (107.96531791909,-7.80924855492) .. (114.03468208095,-7.80924855492)
  .. controls (115.69364161852,-7.80924855492) and (117.27167630060,-7.48554913295) .. (118.24277456650,-6.91907514451)
  -- (118.00000000002,-5.94797687862)
  -- (117.55491329482,-5.94797687862)
  .. controls (116.50289017343,-5.94797687862) and (114.52023121389,-5.17919075145) .. (112.61849710985,-3.19653179191)
  .. controls (111.64739884395,-2.18497109827) and (110.75722543354,-1.13294797688) .. (110.19075144510,-0.08092485549)
  .. controls (116.30057803470,1.49710982659) and (119.37572254338,6.51445086706) .. (119.37572254338,14.00000000001)
  .. controls (119.37572254338,23.14450867054) and (114.84393063586,28.60693641621) .. (105.53757225435,28.60693641621)
  -- cycle;
\path[fill=QKBrandPrimary]
  (124.75722543356,3.52023121388)
  .. controls (124.75722543356,1.82080924856) and (124.43352601159,1.65895953757) .. (122.12716763009,1.53757225434)
  -- (122.12716763009,0.00000000000)
  -- (133.49710982663,0.00000000000)
  -- (133.49710982663,1.53757225434)
  .. controls (131.19075144512,1.65895953757) and (130.86705202316,1.82080924856) .. (130.86705202316,3.52023121388)
  -- (130.86705202316,20.06936416187)
  -- (130.58381502894,20.31213872834)
  -- (122.36994219656,19.13872832372)
  -- (122.36994219656,17.68208092487)
  -- (123.78612716766,17.47976878614)
  .. controls (124.43352601159,17.39884393065) and (124.75722543356,17.03468208094) .. (124.75722543356,15.41618497111)
  -- cycle
  (127.58959537576,22.05202312141)
  .. controls (129.81502890177,22.05202312141) and (131.31213872836,23.67052023123) .. (131.31213872836,25.61271676303)
  .. controls (131.31213872836,27.51445086708) and (129.89595375726,29.13294797690) .. (127.58959537576,29.13294797690)
  .. controls (125.32369942200,29.13294797690) and (123.90751445090,27.51445086708) .. (123.90751445090,25.61271676303)
  .. controls (123.90751445090,23.67052023123) and (125.32369942200,22.05202312141) .. (127.58959537576,22.05202312141)
  -- cycle;
\path[fill=QKBrandPrimary]
  (156.43930635844,2.06358381503)
  .. controls (155.91329479775,2.02312138728) and (155.10404624283,2.06358381503) .. (154.49710982665,2.26589595376)
  .. controls (153.97109826595,2.42774566474) and (153.20231213878,2.91329479769) .. (153.20231213878,5.30057803469)
  -- (153.20231213878,14.64739884394)
  .. controls (153.20231213878,17.15606936418) and (152.79768786133,20.31213872834) .. (145.63583815034,20.31213872834)
  .. controls (139.68786127172,20.31213872834) and (136.04624277461,17.96531791909) .. (136.04624277461,15.33526011562)
  .. controls (136.04624277461,13.51445086706) and (138.63583815033,12.78612716764) .. (139.68786127172,12.78612716764)
  .. controls (140.57803468213,12.78612716764) and (141.02312138733,13.43352601157) .. (141.34682080929,14.40462427747)
  .. controls (142.47976878617,17.84393063585) and (143.77456647404,18.45086705204) .. (144.90751445091,18.45086705204)
  .. controls (146.08092485554,18.45086705204) and (147.25433526017,17.76300578036) .. (147.25433526017,15.45664739886)
  -- (147.25433526017,13.31213872834)
  .. controls (145.83815028907,12.34104046244) and (142.43930635843,11.32947976880) .. (139.80924855496,10.43930635839)
  .. controls (136.61271676305,9.34682080926) and (135.52023121391,7.68786127168) .. (135.52023121391,5.38150289018)
  .. controls (135.52023121391,2.34682080925) and (137.54335260120,-0.48554913295) .. (141.63005780351,-0.48554913295)
  .. controls (144.21965317924,-0.48554913295) and (146.00000000005,0.93063583815) .. (147.41618497115,1.86127167630)
  .. controls (147.94219653184,0.60693641619) and (148.63005780352,-0.48554913295) .. (150.57225433531,-0.48554913295)
  .. controls (152.67630057809,-0.48554913295) and (155.22543352607,0.20231213873) .. (156.56069364168,0.72832369942)
  -- cycle
  (147.25433526017,5.42196531792)
  .. controls (147.17341040467,3.23699421966) and (145.83815028907,2.67052023122) .. (144.74566473993,2.67052023122)
  .. controls (143.16763005785,2.67052023122) and (141.75144508675,3.92485549133) .. (141.75144508675,6.06936416185)
  .. controls (141.75144508675,7.97109826590) and (142.39884393068,8.90173410405) .. (143.61271676305,9.58959537573)
  .. controls (144.86705202317,10.27745664741) and (146.28323699427,10.84393063585) .. (147.25433526017,11.28901734105)
  -- cycle;
\path[fill=QKBrandPrimary]
  (178.69364161857,14.08092485550)
  .. controls (178.65317919083,17.88439306360) and (176.75144508678,20.31213872834) .. (172.58381502897,20.31213872834)
  .. controls (170.23699421972,20.31213872834) and (168.33526011568,19.09826589597) .. (165.66473988446,17.52023121389)
  -- (165.13872832376,20.31213872834)
  -- (157.16763005786,19.13872832372)
  -- (157.16763005786,17.68208092487)
  -- (158.58381502896,17.47976878614)
  .. controls (159.23121387289,17.39884393065) and (159.55491329486,17.03468208094) .. (159.55491329486,15.41618497111)
  -- (159.55491329486,3.52023121388)
  .. controls (159.55491329486,1.82080924856) and (159.23121387289,1.65895953757) .. (156.92485549139,1.53757225434)
  -- (156.92485549139,0.00000000000)
  -- (167.80924855498,0.00000000000)
  -- (167.80924855498,1.53757225434)
  -- (166.95953757232,1.61849710983)
  .. controls (166.10982658966,1.69942196532) and (165.66473988446,1.90173410405) .. (165.66473988446,3.23699421966)
  -- (165.66473988446,12.82658959539)
  .. controls (165.66473988446,13.71676300579) and (165.78612716770,14.64739884394) .. (166.06936416192,15.21387283238)
  .. controls (166.59537572261,16.26589595377) and (167.68786127174,17.19653179192) .. (169.38728323706,17.19653179192)
  .. controls (171.45086705209,17.19653179192) and (172.50289017348,15.94219653181) .. (172.58381502897,13.51445086706)
  -- (172.58381502897,3.23699421966)
  .. controls (172.58381502897,1.90173410405) and (172.13872832377,1.69942196532) .. (171.28901734111,1.61849710983)
  -- (170.43930635845,1.53757225434)
  -- (170.43930635845,0.00000000000)
  -- (181.32369942204,0.00000000000)
  -- (181.32369942204,1.53757225434)
  .. controls (179.01734104054,1.65895953757) and (178.69364161857,1.82080924856) .. (178.69364161857,3.52023121388)
  -- cycle;
\path[fill=QKBrandPrimary]
  (191.19653179200,29.78034682084)
  -- (190.91329479778,30.02312138731)
  -- (182.69942196540,28.93063583818)
  -- (182.69942196540,27.47398843933)
  -- (184.11560693650,27.23121387286)
  .. controls (184.76300578043,27.10982658962) and (185.08670520239,26.74566473991) .. (185.08670520239,25.12716763008)
  -- (185.08670520239,3.52023121388)
  .. controls (185.08670520239,1.82080924856) and (184.76300578043,1.65895953757) .. (182.45664739892,1.53757225434)
  -- (182.45664739892,0.00000000000)
  -- (193.82658959547,0.00000000000)
  -- (193.82658959547,1.53757225434)
  .. controls (191.52023121396,1.65895953757) and (191.19653179200,1.82080924856) .. (191.19653179200,3.52023121388)
  -- (191.19653179200,10.27745664741)
  -- (191.27745664749,10.27745664741)
  .. controls (192.65317919084,7.60693641619) and (194.27167630067,4.85549132948) .. (196.13294797697,2.38728323700)
  .. controls (197.54913294807,0.52601156069) and (199.16763005790,0.00000000000) .. (202.12138728333,0.00000000000)
  -- (205.76300578045,0.00000000000)
  -- (205.76300578045,1.29479768786)
  .. controls (204.91329479779,1.61849710983) and (204.38728323709,2.10404624278) .. (203.17341040472,3.47976878613)
  .. controls (200.46242774576,6.51445086706) and (198.19653179200,9.67052023122) .. (196.05202312148,13.06936416186)
  -- (196.94219653189,13.95953757227)
  .. controls (199.08670520241,16.02312138730) and (201.55491329489,17.80346820811) .. (204.95375722553,18.53179190753)
  -- (204.95375722553,19.82658959539)
  -- (199.08670520241,19.82658959539)
  .. controls (198.19653179200,19.82658959539) and (197.42774566483,19.50289017343) .. (196.69942196541,18.61271676302)
  .. controls (195.93063583824,17.60115606938) and (195.12138728333,16.42774566475) .. (194.19075144518,15.13294797689)
  -- (191.27745664749,11.00578034683)
  -- (191.19653179200,11.00578034683)
  -- cycle;
\path[fill=QKBrandPrimary]
  (221.90751445098,0.00000000000)
  -- (230.32369942209,0.00000000000)
  -- (230.32369942209,1.53757225434)
  .. controls (228.01734104058,1.65895953757) and (227.69364161862,1.82080924856) .. (227.69364161862,3.52023121388)
  -- (227.69364161862,20.06936416187)
  -- (227.41040462440,20.31213872834)
  -- (219.19653179202,19.13872832372)
  -- (219.19653179202,17.68208092487)
  -- (220.61271676312,17.47976878614)
  .. controls (221.26011560705,17.39884393065) and (221.58381502902,17.03468208094) .. (221.58381502902,15.41618497111)
  -- (221.58381502902,6.87861271677)
  .. controls (221.58381502902,6.19075144509) and (221.50289017353,5.21965317920) .. (221.26011560705,4.61271676301)
  .. controls (220.89595375734,3.68208092486) and (219.84393063595,2.71098265896) .. (218.06358381514,2.71098265896)
  .. controls (215.91907514462,2.71098265896) and (214.66473988450,3.96531791908) .. (214.66473988450,7.12138728324)
  -- (214.66473988450,20.06936416187)
  -- (214.38150289028,20.31213872834)
  -- (206.16763005790,19.13872832372)
  -- (206.16763005790,17.68208092487)
  -- (207.58381502900,17.47976878614)
  .. controls (208.23121387294,17.39884393065) and (208.55491329490,17.03468208094) .. (208.55491329490,15.41618497111)
  -- (208.55491329490,5.58381502891)
  .. controls (208.55491329490,0.84971098266) and (211.50867052034,-0.48554913295) .. (214.42196531803,-0.48554913295)
  .. controls (217.86127167641,-0.48554913295) and (219.96531791919,1.37572254335) .. (221.58381502902,2.26589595376)
  -- cycle;
\path[fill=QKBrandPrimary]
  (253.50867052037,14.08092485550)
  .. controls (253.46820809263,17.88439306360) and (251.56647398858,20.31213872834) .. (247.39884393077,20.31213872834)
  .. controls (245.05202312152,20.31213872834) and (243.15028901747,19.09826589597) .. (240.47976878626,17.52023121389)
  -- (239.95375722556,20.31213872834)
  -- (231.98265895966,19.13872832372)
  -- (231.98265895966,17.68208092487)
  -- (233.39884393076,17.47976878614)
  .. controls (234.04624277469,17.39884393065) and (234.36994219666,17.03468208094) .. (234.36994219666,15.41618497111)
  -- (234.36994219666,3.52023121388)
  .. controls (234.36994219666,1.82080924856) and (234.04624277469,1.65895953757) .. (231.73988439319,1.53757225434)
  -- (231.73988439319,0.00000000000)
  -- (242.62427745678,0.00000000000)
  -- (242.62427745678,1.53757225434)
  -- (241.77456647412,1.61849710983)
  .. controls (240.92485549146,1.69942196532) and (240.47976878626,1.90173410405) .. (240.47976878626,3.23699421966)
  -- (240.47976878626,12.82658959539)
  .. controls (240.47976878626,13.71676300579) and (240.60115606950,14.64739884394) .. (240.88439306372,15.21387283238)
  .. controls (241.41040462441,16.26589595377) and (242.50289017354,17.19653179192) .. (244.20231213886,17.19653179192)
  .. controls (246.26589595389,17.19653179192) and (247.31791907528,15.94219653181) .. (247.39884393077,13.51445086706)
  -- (247.39884393077,3.23699421966)
  .. controls (247.39884393077,1.90173410405) and (246.95375722557,1.69942196532) .. (246.10404624291,1.61849710983)
  -- (245.25433526025,1.53757225434)
  -- (245.25433526025,0.00000000000)
  -- (256.13872832384,0.00000000000)
  -- (256.13872832384,1.53757225434)
  .. controls (253.83236994234,1.65895953757) and (253.50867052037,1.82080924856) .. (253.50867052037,3.52023121388)
  -- cycle;
\path[fill=QKBrandPrimary]
  (257.51445086720,28.00000000002)
  -- (257.51445086720,26.46242774569)
  .. controls (260.38728323714,26.34104046245) and (260.71098265911,26.13872832372) .. (260.71098265911,24.07514450869)
  -- (260.71098265911,10.19653179192)
  .. controls (260.71098265911,6.87861271677) and (260.67052023136,5.30057803469) .. (260.50867052038,3.88439306359)
  .. controls (260.38728323714,2.46820809249) and (259.98265895969,1.86127167630) .. (259.05202312153,1.73988439307)
  -- (257.63583815044,1.53757225434)
  -- (257.63583815044,0.00000000000)
  -- (267.38728323715,0.00000000000)
  -- (267.38728323715,1.53757225434)
  -- (265.12138728339,1.73988439307)
  .. controls (263.98843930651,1.82080924856) and (263.54335260131,2.46820809249) .. (263.42196531807,3.88439306359)
  .. controls (263.26011560709,5.34104046243) and (263.21965317934,6.87861271677) .. (263.21965317934,10.19653179192)
  -- (263.21965317934,22.57803468210)
  -- (263.38150289032,22.57803468210)
  .. controls (268.35838150305,15.05202312140) and (273.25433526028,7.52601156070) .. (278.06936416201,0.00000000000)
  -- (282.52023121404,0.00000000000)
  -- (282.52023121404,17.80346820811)
  .. controls (282.52023121404,21.12138728326) and (282.56069364179,22.69942196534) .. (282.72254335277,24.11560693644)
  .. controls (282.84393063601,25.53179190754) and (283.24855491346,26.13872832372) .. (284.17919075161,26.26011560696)
  -- (285.59537572271,26.46242774569)
  -- (285.59537572271,28.00000000002)
  -- (275.84393063600,28.00000000002)
  -- (275.84393063600,26.46242774569)
  -- (278.10982658976,26.26011560696)
  .. controls (279.24277456664,26.17919075147) and (279.68786127184,25.53179190754) .. (279.80924855508,24.11560693644)
  .. controls (279.97109826606,22.65895953759) and (280.01156069381,21.12138728326) .. (280.01156069381,17.80346820811)
  -- (280.01156069381,8.73988439307)
  -- (279.84971098282,8.73988439307)
  .. controls (275.56069364178,15.17341040464) and (271.27167630074,21.56647398846) .. (267.10404624293,28.00000000002)
  -- cycle;
\path[fill=QKBrandPrimary]
  (303.84393063602,6.23121387284)
  .. controls (302.63005780365,3.92485549133) and (300.89017341059,2.63005780347) .. (298.42196531810,2.63005780347)
  .. controls (294.37572254353,2.63005780347) and (293.00000000018,5.94797687862) .. (293.00000000018,10.19653179192)
  -- (303.43930635857,10.19653179192)
  .. controls (304.89595375741,10.19653179192) and (305.62427745684,10.60115606937) .. (305.62427745684,11.89595375724)
  .. controls (305.62427745684,15.21387283238) and (304.36994219672,20.31213872834) .. (296.56069364180,20.31213872834)
  .. controls (289.27745664757,20.31213872834) and (286.56647398861,15.57803468209) .. (286.56647398861,9.91329479770)
  .. controls (286.56647398861,4.41040462428) and (288.95375722561,-0.52601156069) .. (296.47976878631,-0.48554913295)
  .. controls (301.29479768805,-0.48554913295) and (303.92485549152,1.86127167630) .. (305.30057803487,5.42196531792)
  -- cycle
  (293.00000000018,12.13872832371)
  .. controls (293.00000000018,15.05202312140) and (293.76878612735,18.45086705204) .. (296.39884393082,18.45086705204)
  .. controls (298.86705202330,18.45086705204) and (299.27167630076,15.37572254337) .. (299.27167630076,13.47398843932)
  .. controls (299.27167630076,12.38150289018) and (298.94797687879,12.13872832371) .. (298.01734104064,12.13872832371)
  -- cycle;
\path[fill=QKBrandPrimary]
  (320.15028901754,17.80346820811)
  -- (320.15028901754,19.82658959539)
  -- (315.94219653199,19.82658959539)
  -- (315.94219653199,24.92485549135)
  -- (313.59537572274,24.92485549135)
  -- (310.03468208112,19.82658959539)
  -- (307.48554913314,19.82658959539)
  -- (307.48554913314,17.80346820811)
  -- (309.83236994239,17.80346820811)
  -- (309.83236994239,4.73410404625)
  .. controls (309.83236994239,1.05202312139) and (312.58381502910,-0.48554913295) .. (314.84971098285,-0.48554913295)
  .. controls (316.50867052043,-0.48554913295) and (319.01734104066,0.28323699422) .. (321.28323699442,1.69942196532)
  -- (320.83815028922,2.95375722544)
  .. controls (320.27167630078,2.71098265896) and (319.42196531812,2.54913294798) .. (318.53179190771,2.54913294798)
  .. controls (316.99421965338,2.54913294798) and (315.94219653199,3.68208092486) .. (315.94219653199,6.27167630058)
  -- (315.94219653199,17.80346820811)
  -- cycle;


==> assets/qiankunnet-symbol-paths.tex <==
% Exact vector contours from the user-supplied VI v0.3 outlined SVG.
% Units are those of the master: cap height 28; baseline y=0.
% No font file, raster artwork or shell escape is required.
\fill[QKBrandPrimary] (0,23.2) rectangle (36,28);
\fill[QKBrandPrimary] (0,11.6) rectangle (36,16.4);
\fill[QKBrandPrimary] (0,8.88178e-16) rectangle (36,4.8);
\fill[QKBrandSecondary] (42,23.2) rectangle (57,28);
\fill[QKBrandSecondary] (42,11.6) rectangle (57,16.4);
\fill[QKBrandSecondary] (42,8.88178e-16) rectangle (57,4.8);
\fill[QKBrandSecondary] (63,23.2) rectangle (78,28);
\fill[QKBrandSecondary] (63,11.6) rectangle (78,16.4);
\fill[QKBrandSecondary] (63,8.88178e-16) rectangle (78,4.8);

